Stochastic Parameter Prediction in Cardiovascular Problems

Patient-specific modeling of cardiovascular flows with high-fidelity is challenging due to its dependence on accurately estimated velocity boundary profiles, which are essential for precise simulations and directly influence wall shear stress calculations - key in predicting cardiovascular diseases like atherosclerosis. This data, often derived from in vivo modalities like 4D flow MRI, suffers from low resolution and noise. To address this, we employ a stochastic data assimilation technique that integrates computational fluid dynamics with an advanced Ensemble-based Kalman filter, enhancing model accuracy while accounting for uncertainties. Our approach sequentially collects velocity data over time within the vascular model, enabling real-time refinement of unknown boundary estimations. The mathematical model uses the incompressible Navier-Stokes equation to simulate aortic blood flow. We consider unknown boundaries as constant, time-dependent, and space-time dependent in two- and three-dimensional models. In our 2-dimensional model, relative errors were as low as 0.996\% for constant boundaries and up to 2.63\% and 2.61\% for time-dependent and space-time dependent boundaries, respectively, over an observation span of two-time steps. For the 3-dimensional patient-specific model, the relative error was 7.37\% for space-time dependent boundaries. By refining the velocity boundary profile, our method improves wall shear stress predictions, enhancing the accuracy and reliability of models specific to individual cardiovascular patients. These advancements could contribute to better diagnosis and treatment of cardiovascular diseases.

==> sections/IntroSajad.tex <==
\section{Introduction}\label{sec:Intro}

In a clinical context, in vivo methods generally rely on non-invasive imaging techniques, such as ultrasound or magnetic resonance imaging (MRI), to estimate blood flow velocities and vessel geometries \citep{agbalessi2023tracking}. But, in vivo measurements of wall shear stress (WSS), which is crucial for anticipating cardiovascular diseases like atherosclerosis, are difficult to capture directly through standard clinical methods \citep{urschel2021investigation}. Thus, engaging with simulations of a complex cardiovascular system leads to prediction capabilities that cannot be attained only based on in-vivo tests \citep{peirlinck2021precision}. \\

It is common practice in clinical settings to estimate blood flow velocities and vessel geometries using non-invasive imaging techniques like ultrasound or magnetic resonance imaging (MRI) when using in vivo methods \citep{agbalessi2023tracking}. Unfortunately, conventional clinical methods have a hard time directly measuring in vivo wall shear stress (WSS), an important factor in predicting cardiovascular diseases such as atherosclerosis \citep{urschel2021investigation}. Thus, the ability to make predictions that cannot be achieved solely through in-vivo tests is gained by participating in simulations of intricate cardiovascular systems \citep{peirlinck2021precision}.\\


Computational cardiology is a multi-disciplinary field that has seen extensive progress in the past decade \citep{kashtanova2023simultaneous, bai2023diagnosis}. In particular, recent advances in numerical analysis, computational resources, and the development of patient-specific models, known as digital twins, have allowed researchers to address critical challenges related to limitations of clinical methods \citep{de2022evidence}. In this regard, the hemodynamics simulations have proven helpful for planning and assessing life-threatening cardiovascular pathologies, including aortic dissection \citep{wu2023vitro}, stenosis \citep{nadeem2023numerical}, and aneurysms \citep{salavatidezfouli2024effect}, which are known to be highly affected by blood flow patterns. 

Hemodynamic modeling based on varying complexity ranges from lumped models that are electric analogues of the circulation, through one-dimensional (1D) Euler equations and three-dimensional (3D) Navier–Stokes models, to geometrical multi-scale models have been developed to study various healthy and diseased physiologies \citep{pant2017inverse}. As a common point, all mentioned methods need to be provided with necessary model parameters such as blood properties and inflow/outflow boundary conditions \citep{armour2021influence}. The most common way to obtain boundary parameters is based on Phase Contrast Magnetic Resonance Imaging (PC-MRI) \citep{stankovic20144d}, a medical imaging modality developed with the aim of visualizing and quantifying the blood flow in the vasculature \citep{martin20242115}. In the literature, this imaging technique is also called 4D PC-MRI or 4D-flow MRI, because it includes time-resolved slice images covering a volume of acquisition, with flow encoding \citep{zhuang2021role}. It provides both anatomical (magnitude images) and functional (phase images) information that enables the non-invasive analysis of blood hemodynamics in the vessel \citep{morgan20214d}. 

However, 4D-flow analysis for generation of the velocity profile in a section of the vessel requires extensive pre-processing \citep{agbalessi2023tracking}. In particular, the extraction of the aortic properties at each time step of the cardiac cycle may be needed \citep{tahoces2019automatic}. Moreover, data associated with 4D MRI is of noisy (uncertainty) nature which necessitates separate pre-processing \citep{de2020data}. Hence, the exact estimation of model parameters and inclusively boundary profile of the vascular system is still a matter of question \citep{arthurs2020flexible}. Data assimilation techniques are intended to solve this limitation by incorporating distributed in-vivo or in-vitro data \citep{bertoglio2014identification}.  

In recent years, the data assimilation approach has gained popularity as it can take advantage of full-time varying measurements to adjust the parameters and states of models in real time, enhancing the accuracy and reliability of forecasts and simulations in various fields such as meteorology, oceanography, and hydrology \citep{lim2023data}. This method effectively integrates observational data with model predictions to reduce uncertainties and improve decision-making processes \citep{de2021data}. It has been employed in a range of cardiovascular problems such as the estimation of Windkessel parameters \citep{fevola2023vector}, closed-loop lumped model parameters for single-ventricle physiology \citep{bjordalsbakke2022parameter}, artery wall stiffness parameters \citep{imperiale2021sequential} and tissue support parameters for fluid-structure interaction models \citep{shidhore2022estimating}.

Many previous studies have tackled the inverse problem, with a focus on estimating parameters that define the boundary conditions of the model. For a review of their pros and cons, see references \citep{arbia2015pulmonary, perdikaris2016model, fevola2022boundary, SmithThesis}. Recently, a Bayesian method for this kind of parameter estimation in cardiovascular models has been developed, utilizing Markov chain Monte Carlo (MCMC) methods to target mean or maximum values, as discussed in reference \citep{Schiavazzi2017Patient}. In contrast to these methods, the Kalman filter (KF) offers a flexible and computationally efficient approach for parameter estimation in complex systems, dynamically integrating observational data with predictive models to improve accuracy over time \citep{Canuto2020AnEK}. Kalman filter variants are sequential data assimilation techniques that correct the computed state and model parameter estimates at each simulation time step. These corrections account for the error between available measurements and current numerical predictions \citep{Walia2023PPGbasedWM}.

In this paper, a method for parameter estimation for patient-specific cardiovascular models is described and tested. The underlying estimation technique is the ensemble Kalman filter (EnKF), originally developed for data assimilation into dynamical models for numerical weather forecasting \citep{Fang2017EnsemblebasedSI}. The primary advantage of the EnKF is its applicability to such nonlinear dynamical systems. While other parameter estimation techniques exist for cardiovascular models \citep{Canuto2020AnEK}, to the best of the authors' knowledge, there is no similar work reported in the literature for high fidelity vascular models, primarily owing to difficulties in implementation, handling model dynamics, and computational demands. 

\begin{itemize}
    \item Using 2 dimension high fidelity solver in forward problem of filter
    \item Investigating different types of velocity boundary condition such as constant, time dependent and time-space dependent velocity boundary condition.
    \item I should improve those bullet points and add some other 
\end{itemize}
